On Optimizing the Conditional Value-at-Risk of a Maximum Cost for Risk-Averse Safety Analysis

The popularity of Conditional Value-at-Risk (CVaR), a risk functional from finance, has been growing in the control systems community due to its intuitive interpretation and axiomatic foundation. We consider a nonstandard optimal control problem in which the goal is to minimize the CVaR of a maximum random cost subject to a Borel-space Markov decision process. The objective represents the maximum departure from a desired operating region averaged over a given fraction of the worst cases. This problem provides a safety criterion for a stochastic system that is informed by both the probability and severity of the potential consequences of the system's behavior. In contrast, existing safety analysis frameworks apply stage-wise risk constraints or assess the probability of constraint violation without quantifying the potential severity of the violation. To the best of our knowledge, the problem of interest has not been solved. To solve the problem, we propose and study a family of stochastic dynamic programs on an augmented state space. We prove that the optimal CVaR of a maximum random cost enjoys an equivalent representation in terms of the solutions to these dynamic programs under appropriate assumptions. For each dynamic program, we show the existence of an optimal policy that depends on the dynamics of an augmented state under the assumptions. In a numerical example, we illustrate how our safety analysis framework is useful for assessing the severity of combined sewer overflows under precipitation uncertainty.

==> 5_numerical_example.tex <==

\textcolor{blue}{Risk-averse safety analysis, as presented here, suffers from the curse of dimensionality inherent to DP and requires an augmented state space. Despite these computational challenges, risk-averse safety analysis may be a useful tool for designing control systems. At the design stage, large-scale off-line simulations may be commonplace, and designers may be required to assess multiple alternatives in light of uncertainty.}

%Risk-averse safety analysis requires off-line computations. While these computations suffer from the curse of dimensionality (due to DP and the augmented state space), designing systems often requires large-scale off-line simulations computations. We see risk-averse safety analysis as a tool help practitioners evaluate which design changes to a control system may be more appropriate under uncertainty.

We consider the task of modifying the design of an urban stormwater system. We refer the reader to \cite{extendedversion} for more details about the simulation setting. %While stormwater assets vary widely in practice, the system that we consider has some typical attributes.%
%Apart from being actively controlled, the stormwater system that we consider is otherwise typical.\footnote{Actively controlled stormwater systems are becoming more common but are relatively novel technologies (e.g., see \cite{smartwater}).} 
%trying to frame it as a ``novel'' technology
%still represent a relatively new technology. most stormwater systems are passive. While our safety analysis method applies to passive systems, its application to an actively controlled system demonstrates its ability to assess the performance of different actuators (e.g., valve versus pump).
The system consists of two tanks (tank 1, tank 2) connected by an automated valve. Water flows by gravity between the tanks based on the relative difference in water levels and the position of the valve. Water enters the system through a random process of surface runoff. Water exits the system through a \emph{storm sewer} drain that is connected to tank 2 or through outlets that lead to a \emph{combined sewer}. %A combined sewer allows a combination of stormwater and untreated wastewater to discharge into natural waterways when there is too much surface runoff to collect.% 
The storm sewer directs stormwater to a nearby water body, which occurs without penalty. However, the storm sewer's capacity is limited. When water levels are too great, excess flows are directed to a combined sewer, which can release a mixture of stormwater and untreated wastewater into a local waterway. 
%In drier periods, a combined sewer carries a mixture of untreated wastewater and stormwater to a wastewater treatment plant. However, when storm events cause the flow in a combined sewer to exceed its design capacity, a flow regulator (downstream from our system) will divert some of the untreated mixture of stormwater and sewage into a nearby water body. 
This event is called a \emph{combined sewer overflow} (CSO), which can disturb local ecosystems. %Combined sewers are present in older cities, such as Toronto and San Francisco, and overflows from these sewers can harm local ecosystems. 
We apply risk-averse safety analysis to examine how design modifications may reduce the risk of CSOs by managing the system's maximum water levels. The designs are: a) baseline, b) replace the valve with a controllable bidirectional pump, and c) retrofit tank 1 with an outlet that drains to a storm sewer without penalty.

%
%\begin{figure*}[ht]
%\centerline{\includegraphics[width=\textwidth]{watersys_baseline.png}}
%\caption{A schematic of the stormwater system and a probability mass function for the surface runoff disturbance (cubic feet per second, cfs). The baseline design and three alternative designs are shown.}
%\label{watersysdrawing}
%\end{figure*}
%\textcolor{orange}{Can we place the dotted line at the bottom of the red circles? I think that is more accurate if it is meant to indicate the water level at which the water starts discharging to the combined sewer. -KMS}
%\subsubsection{System model for baseline design} 

$X_t = [X_{t1}, X_{t2}]^T$ is the vector of random water levels in tank 1 and tank 2 at time $t$. The state space is $S = [0, \bar{k}_1] \times [0, \bar{k}_2]$ ft\textsuperscript{2}, where $\bar{k}_i = k_i + 2$ ft and $k_i$ is the maximum water level that tank $i$ can hold without releasing water into the combined sewer. The desired operating region is $K = [0, k_1] \times [0, k_2]$. We choose $c_t = g_K$ for every $t \in \mathbb{T}_N$, where $g_K(x) = \max\{x_{1} - k_1, x_{2} - k_2, 0\}$ quantifies the maximum water elevation outside $K$. For the baseline design, the control input is the valve position at time $t$, and the control space is $C = [0,1]$ (closed to open, unitless). The tuple $(W_0,W_1,\dots,W_{N-1})$ is a random process of surface runoff that arises due to precipitation uncertainty (units: ft\textsuperscript{3}/s). We select a disturbance distribution to reflect simulations from our prior work \cite{sustech}. We use Newtonian physics and a mass balance to form a dynamics function $(f = f_t \;\;  \forall t \in \mathbb{T})$ for each design. We consider $N=20$; $[t,t+1)$ represents a duration of 3 minutes. $\hat{\mathcal{S}}$ denotes a computation of a set $\mathcal{S}$.

%$W_t$ and $W_\tau$ are independent for all $t \neq \tau$ and do not depend on the current state or control in this example. The notation $\triangle \tau$ denotes the duration between time $t$ and time $t+1$, which is constant for all $t \in \mathbb{T}$.
%\textcolor{orange}{We chose to make the disturbances i.i.d. for simplicity right? \textcolor{blue}{yes} What are the real requirements for the algorithm? I think we need for the disturbances to be independent, but not necessarily identically distributed? \textcolor{blue}{yes this is correct} For example, we could draw from a different distribution at each timestep, but those draws must be independent of draws in other timesteps. Is this correct? \textcolor{blue}{yes this is correct}  Just thinking about what we want to emphasize here. -KMS \textcolor{blue}{what do you think of the revision?}} 

%Let $t \in \mathbb{T}$ be given. If $x_t \in S$, $u_t \in A$, and $w_t \in \mathbb{R}$ are the values of $X_t$, $U_t$, and $W_t$, respectively, then the value of $X_{t+1}$ is given by
%\begin{subequations}\label{dynwater}
%\begin{equation}\begin{aligned}
%    x_{t+1} = x_t + f_0(x_t,u_t,w_t)\cdot \triangle\tau,
%\end{aligned}\end{equation}
%such that if $x_{t+1,i} \geq \overline{k}_i$, then we redefine $x_{t+1,i} \coloneqq \overline{k}_i$.
%\begin{equation}\begin{aligned}
%    x_{t+1} & = f(x_t,u_t,w_t) \\
%    & = \min\left\{\max\left\{x_t + f_0(x_t,u_t,w_t)\cdot \triangle\tau,  \begin{bmatrix} 0 \\0 \end{bmatrix}\right\}, \begin{bmatrix}\;\overline{k}_1 \\ \;\overline{k}_2\end{bmatrix} \right\}.
%\end{aligned}\end{equation}
%The above equation means that if the quantity $x_t + f_0(x_t,u_t,w_t)\cdot \triangle\tau$ is in $S$, then $x_{t+1} = x_t + f_0(x_t,u_t,w_t)\cdot \triangle\tau$. Otherwise, the value $x_t + f_0(x_t,u_t,w_t)\cdot \triangle\tau$ is truncated so that $x_{t+1}$ is in $S$. This is a standard technique for implementing dynamic programming on a non-linear system. 
%
%The function $f_0 : \mathbb{R}_+^2 \times A \times \mathbb{R} \rightarrow \mathbb{R}_+^2$ is chosen according to simplified Newtonian physics:
%\begin{equation}\label{physics}\begin{aligned}
%f_0(x,u,w) & \coloneqq \left[ f_{01}(x,u,w), f_{02}(x,u,w) \right]^{T},\\
%f_{01}(x,u,w) & \coloneqq  \frac{w - q_{\text{cso,1}}(x) - q_\text{valve}(x,u)}{a_1},\\
%f_{02}(x,u,w) & \coloneqq  \frac{w - q_{\text{cso,2}}(x) + q_\text{valve}(x,u)  - q_\text{storm,2}(x)}{a_2}, \\
%q_\text{valve}(x,u) & \coloneqq u \cdot \tilde{\pi} r_\text{v}^2 \cdot \text{sign }{h(x)} \cdot \sqrt{2 \tilde{g} |h(x)|},  \\
%h(x) & \coloneqq \max(x_1 - z_1,0) - \max(x_2 - z_{1,\text{in}},0).\\
%q_\text{storm,2}(x) &:= \begin{cases} c_\text{d} \bar{\pi} r_\text{d}^2 \sqrt{2 \tilde{g} (x_2 - z_2)} & \text{if } x_2 \geq z_2 \\0 & \text{otherwise} \end{cases}.
%\end{aligned}\end{equation}
%
%Table \ref{tanksysinfo} lists model parameters. The outlets to the combined sewer and to the storm sewer are equipped with outflow regulation devices that produce a linear outflow rate. For example, $q_\text{storm,2}(x)$ with $x \in S$ is given by
%\begin{equation}\label{stormq}
   %q_\text{storm,2}(x) \coloneqq q_\text{max,2} - \frac{q_\text{max,2}}{\overline{k}_2 - z_{2}} \min\{\overline{k}_2-x_2, %\overline{k}_2 - z_{2}\},
%\end{equation}
%\end{subequations}
%where $q_\text{max,2} \coloneqq c_\text{d} \tilde{\pi} r_{\text{s}}^2 \big(2 \tilde{g} (\overline{k}_2 - z_2)\big)^{\frac{1}{2}}$ is tank 2's maximum outflow rate to the storm sewer, $c_\text{d}$ is a discharge coefficient, $\tilde{\pi} \approx 3.14$, $\tilde{g}$ is gravitational acceleration, $r_{\text{s}}$ is the storm sewer outlet radius, and $z_{2}$ is the storm sewer outlet elevation. The outflow rates to the combined sewer, $q_{\text{cso,1}}$ and $q_{\text{cso,2}}$, are defined similarly to \eqref{stormq}. 
%We show this function in the left panel of Fig.~\ref{exgk}.

%\begin{table}[ht]
%\caption{Stormwater System Parameters (Baseline)}
%\label{table}
%\setlength{\tabcolsep}{3pt}
%\begin{tabular}{|p{25pt}|p{125pt}|p{63pt}|}
%\hline
%\textbf{Symbol} &  \textbf{Description} & \textbf{Value} \vspace{.5mm}\\
%\hline
%$a_1$ & Surface area of tank 1 & 30000 ft\textsuperscript{2} \vspace{.6mm}\\
%$a_2$ & Surface area of tank 2 & 10000 ft\textsuperscript{2} \vspace{.6mm}\\
%
%$c_d$ & Discharge coefficient & 0.61 (no units) \vspace{.6mm}\\
%
%$\tilde{g}$ & Acceleration due to gravity & 32.2 $\frac{\text{ft}}{\text{s}^2}$\vspace{.6mm}\\
%
%$\underline{g}$ & Minimum of $g_K$ & 0 ft\vspace{1mm}\\
%
%$\overline{g}$ & Maximum of $g_K$ & 2 ft\vspace{.6mm}\\
%
%$k_1$ & Combined sewer (cs) outlet elevation, tank 1 & 3 ft \vspace{.6mm}\\
%
%$k_2$ & cs outlet elevation, tank 2 & 4 ft \vspace{.6mm}\\
%
%$\overline{k}_1$ & Maximum value of $x_1$ & 5 ft \vspace{.6mm}\\
%
%$\overline{k}_2$ & Maximum value of $x_2$ & 6 ft \vspace{.6mm}\\
%
%$N$ & Length of discrete time horizon & 20 ($=$ 1 h) \vspace{.6mm}\\
%
%$\tilde{\pi}$ & Circle circumference-to-diameter ratio & $\approx$3.14 \vspace{.6mm}\\
%
%$r_\text{s}$ & Storm sewer outlet radius & $1/3$ ft \vspace{.6mm}\\
%
%$r_\text{v}$ & Valve radius & $1/3$ ft\vspace{.6mm}\\
%
%$ \triangle \tau $ & Duration of $[t,t+1)$ & 3 min \vspace{.6mm}\\
%
%$z_1$ & Pipe elevation w.r.t. tank 1 base & 1 ft\vspace{.6mm}\\
%
%$z_{1,\text{in}}$ & Pipe elevation w.r.t. tank 2 base & 2 ft\vspace{.6mm}\\
%
%$z_2$ & Storm sewer outlet elevation & 1 ft\vspace{.6mm}\\
%
%N/A & Number of cs outlets, tank 1 & 3 \vspace{.6mm}\\
%
%N/A & Number of cs outlets, tank 2 & 1 \vspace{.6mm}\\
%
%N/A & cs outlet radius, tank 1 & 1/4 ft \vspace{.6mm}\\
%
%N/A & cs outlet radius, tank 2 & 3/8 ft \vspace{.5mm}\\
%\hline
%\multicolumn{3}{p{251pt}}{cs $=$ combined sewer, ft $=$ feet, s $=$ 
%seconds, min $=$ minutes, h $=$ hours.}
%\end{tabular}
%\label{tanksysinfo}
%\end{table}

%We use a finite distribution for the disturbance process, which does not depend on the values of the current state or control. In prior work \cite{sustech}, we simulated a design storm in PCSWMM software (Computational Hydraulics International), which is an extension of the US Environmental Protection Agency's Stormwater Management Model \cite{swmm}. A \emph{design storm} is a synthetic precipitation time series based on historical data that a local government uses to specify regulations for new or retrofitted stormwater systems. The empirical distribution from our simulations had positive skew, and the mean was approximately 12.2 cfs. We used these characteristics to inform the choice of the disturbance distribution shown in Fig.~\ref{watersysdrawing}: mean (12.2 cfs), variance (9.9 cfs$^2$), and skew (0.74).
%
%We \textcolor{blue}{identified this distribution in prior work} \cite{chapmantac2021, sustech} by simulating a design storm 
%For each $t$, approximate statistics of the distribution of $W_t$ are: mean (12.2 cfs), variance (9.9 cfs$^2$), and skew (0.74), where cfs is cubic feet per second. 
%[my_mean, my_variance, my_skew] = Get_Empirical_Stat_Disturbance_Profile('right skew')

%\subsubsection{Verification of Assumption \ref{Assumption1}} It holds that $g_K(x) \in [\underline{g},\overline{g}] = [0,2]$ for all $x \in S$, where $g_K$ is defined by \eqref{mygksw}. We choose $c(x,u) = c_N(x) = g_K(x) - \underline{g}$ for all $x \in S$ and $u \in A$. Thus, all values of $c$ and $c_N$ are elements of $\mathcal{Z} \coloneqq [0, \bar{c}] = [0, 2]$, and $c$ and $c_N$ are continuous functions. The control space $A = [0,1]$ is compact. In our example, the stochastic kernel for the disturbance process $p(\mathrm{d}w|x,u)$ does not depend on $(x,u)$, which implies that it is constant and therefore continuous in $(x,u)$. %\footnote{$p(\mathrm{d}w|x,u)$ is a continuous stochastic kernel on $\mathbb{R}$ given $S \times A$ if the function $\gamma : S \times A \rightarrow \mathcal{P}(\mathbb{R})$, $\gamma(x,u) := p(\mathrm{d}w|x,u)$, is continuous.} 
%The dynamics function \eqref{dynwater} is continuous since it is a composition of continuous functions. Recall that the function $\lambda(x) \coloneqq \text{sign}(x) \, \sqrt{\lvert x \rvert}$ is continuous since $\lim_{x \uparrow 0} \lambda(x) = \lim_{x \downarrow 0} \lambda(x) = 0$.
%\subsubsection{Designs} We investigate the effect of different designs on the system's safety, as quantified in terms of risk-sensitive safe sets. The designs are listed below:
%\begin{enumerate}[label=\alph*)] 
 %    \item Baseline;
%    \item Replace the valve with a \textcolor{black}{controllable bidirectional} pump, whose maximum pumping rate is $\overline{q}_{\text{pump}}$;
%    \item Retrofit tank 1 with an outlet that drains to a storm sewer without penalty; or
%    \item Increase the surface area of tank 2 by 20\%.
%\end{enumerate}
%We modify the baseline system model to obtain a model representing design b, c, or d. For design d, we set $a_2 = 12000$ ft\textsuperscript{2}. For design c, the equation for the flow through tank 1 changes to the following:
%\begin{equation}
%    f_{01}(x,u,w)  \coloneqq  \frac{w - q_{\text{cso,1}}(x) - q_\text{valve}(x,u) - q_\text{storm,1}(x)}{a_1},\\
%\end{equation}
%where $q_\text{storm,1}(x)$ takes the same form as $q_\text{storm,2}(x)$ in \eqref{stormq}. 
%For design b, the control space becomes $A = [-1, 1]$, and the term $q_{\text{valve}}(x,u)$ is replaced by $q_\text{pump}(x,u)$, which models the flow rate generated by a pump. Prior to presenting the form of $q_\text{pump}(x,u)$, we introduce its dependencies, $\mathcal{I}_i(x,u)$ and $\ell(x_i,u)$. $\mathcal{I}_i(x,u)$ is a Boolean variable that determines whether the water level is too low to permit pumping, and the function $\ell(x_i,u)$ represents a start-up phase. $\mathcal{I}_1(x,u)$ is true if and only if the pump attempts to push water from tank 1 to tank 2 ($u < 0$), but the water level in tank 1 is too low. $\mathcal{I}_2(x,u)$ has an analogous interpretation. Formally, we define $\mathcal{I}_1(x,u)$ and $\mathcal{I}_2(x,u)$ as follows:
%\begin{subequations}\label{pumpeq}
%\begin{equation}\begin{aligned}
%    \mathcal{I}_1(x,u) & \coloneqq x_1 < z_\text{p} - \epsilon \text{ and } u < 0\\
%    \mathcal{I}_2(x,u) & \coloneqq x_2 < z_\text{p} - \epsilon \text{ and }u \geq 0,
%\end{aligned}\end{equation}
%where $z_\text{p}$ is a threshold elevation and $\epsilon$ is a small positive number. We define the function $\ell(x_i,u)$ as follows:
%\begin{equation}
%    \ell(x_i,u) \coloneqq \frac{\overline{q}_{\text{pump}} \cdot u}{2 \epsilon} (x_i + \epsilon - z_\text{p} ).
%\end{equation}
%We define $q_\text{pump}(x,u)$ as follows:
%\begin{equation}\label{qpump1}
%    q_\text{pump}(x,u) \coloneqq \begin{cases}0 & \text{if }\mathcal{I}_1(x,u) \text{ or } \mathcal{I}_2(x,u) \\ -\ell(x_1,u) & \text{if } x_1 \in [z_\text{p} - \epsilon,z_\text{p} + \epsilon] \text{ and } u < 0\\
%    -\ell(x_2,u) & \text{if } x_2 \in [z_\text{p} - \epsilon,z_\text{p} + \epsilon] \text{ and } u \geq 0\\
%    -u \cdot \overline{q}_{\text{pump}} & \text{otherwise}.\end{cases}
%\end{equation}
%\end{subequations}
%One can show that $q_\text{pump}$ is a composition of continuous functions by replacing the case statements in \eqref{qpump1} with minimum and maximum operators:
%    \begin{align*}
 %       q_\text{pump}(x,u) &= \frac{-\overline{q}_{\text{pump}}}{2 \epsilon} \Bigl( \min\{ 0, u\} \nu(y_1) + \max\{ 0, u\} \nu(y_2) \Bigr) \\
 %       \nu(y) &\coloneqq \max\{ 0 , \min\{y, 2\epsilon \}\} \\
 %       y_i &\coloneqq x_i + \epsilon - z_\text{p}.
 %   \end{align*}
%Table \ref{pumpdesign} lists model parameters for the pump design (b).
%
%\begin{table}[ht]
%\caption{Stormwater System Parameters (Pump design)}
% \label{table}
%\setlength{\tabcolsep}{3pt}
%\begin{tabular}{|p{25pt}|p{125pt}|p{63pt}|}
%\hline
%\textbf{Symbol} &  \textbf{Description} & \textbf{Value} \vspace{.5mm}\\
%\hline
%$\overline{q}_{\text{pump}}$ & Maximum pumping rate & 10 cfs \vspace{.5mm}\\
%$\epsilon$ & Slack variable & $\frac{1}{12}$ ft \vspace{.6mm}\\
%$z_\text{p}$ & Threshold pumping elevation & 1 ft \vspace{.6mm}\\
%\hline
%\multicolumn{3}{p{251pt}}{ft $=$ feet, cfs $=$ 
%cubic feet per second.}
%\end{tabular}
%\label{pumpdesign}
%\end{table}
%

Fig.~\ref{exactvsunderapprox} presents computations of $\mathcal{S}_\alpha^r$ \eqref{13}. For comparison, Fig.~\ref{exactvsunderapprox} also presents computations of the underapproximations $\mathcal{U}_{\alpha,\gamma}^r$ using the method from \cite{chapmantac2021}. As the risk-aversion level $\alpha$ becomes smaller (more pessimistic), the contours of $\hat{\mathcal{S}}_\alpha^r$ and $\hat{\mathcal{U}}_{\alpha,\gamma}^r$ contract, as we expect, while the qualitative features are preserved. The contours for the pump design (b) are more rectangular than those for the baseline design (a). The contours for the outlet design (c) are stretched farther along the $x_1$-axis (tank 1's effective capacity increases) vs. the baseline design.

%using the proare shown in Fig.~\ref{exactvsunderapprox}, which we completed via the procedure outlined in \mbox{Sec.~\ref{keyprocedure}}
%For comparison, we provide computations of the under-approximation set $\mathcal{U}_{\alpha,\gamma}^r$ ($\gamma = 20$), which we completed via the method from our prior work \cite{chapmantac2021}. 
%
%The under-approximation method uses a $\gamma$-dependent soft-maximum and an $\alpha$-dependent upper bound for CVaR to derive a $(\gamma,\alpha)$-dependent upper bound for $W_\alpha^*$ (Def. \ref{salphar}).  The value functions for this MDP problem are defined on the original state space $S$, and the objective is an expected cumulative $\gamma$-dependent cost. We explored values of $\gamma$ between 10 and 120 in increments of roughly 10. We chose $\gamma = 20$ because this value provides relatively large estimates of $\mathcal{U}_{\alpha,\gamma}^r$ for more risk-averse values of $\alpha$. The selection of an appropriate $\gamma$ depends on one's preferences, and additional guidance is provided in \cite{chapmantac2021}.
%When comparing the results for $\gamma = 10$ versus $\gamma = 30$, we observed trade-offs in which the under-approximation sets were larger for some values of $\alpha$ and smaller for other values of $\alpha$, which is our rationale for choosing $\gamma = 20$. 
% 54 hours and 30 cores in total for 4 designs
% 54 hours/4 = about 13.5 hours per design
% The complete job (with four designs) required about 54 hours and 30 CPU cores. 
The underapproximation method \cite{chapmantac2021} requires the manual tuning of a soft-max parameter $\gamma$ that impacts the fidelity of the underapproximation set $\mathcal{U}_{\alpha,\gamma}^r$ at different levels of $\alpha$. The current method provides $\mathcal{S}_\alpha^r$ exactly in principle and does not involve the tuning of an additional parameter, but it does require significantly more resources.\footnote{We provide a rough comparison of resources; we have made no attempt to optimize efficiency beyond parallelizing the operations in a given DP recursion. One can run the underapproximation method on a standard laptop (2-4 CPU cores) in approximately 10 minutes for a fixed $\gamma$ and a fixed design. However, the current method takes about 13.5 hours and 30 CPU cores for a fixed design. We used the Tufts Linux Research Cluster (Medford, MA) running MATLAB (The Mathworks, Inc.). Our code is available from https://github.com/risk-sensitive-reachability/RSSAVSA-2021.} This is due to the augmented state space $\mathbb{S} = S \times \mathcal{Z}$ and solving dynamic programs for different values of the dual parameter $s$. In contrast, for a fixed $\gamma$, solving one MDP problem on $S$ is required to compute $\mathcal{U}_{\alpha,\gamma}^r$ for every $\alpha$ and $r$ of interest \cite{chapmantac2021}.
%Moreover, problems with different dual parameters can be solved in parallel to reduce computation time.
%
%First, due to time inconsistency and a non-additive cost function, the dynamic program that determines the minimum CVaR is solved on an augmented state space, which is the Cartesian product of the original state space $S$ and the interval $\mathcal{Z}$. Moreover, due to the representation of CVaR that our method uses, a second outer optimization over the dual parameter must be solved. Consequently, the inner dynamic program is solved repeatedly with different values of the dual parameter. While this increases the computational complexity significantly, 
% In practice, this means that the inner dynamic program needs to be solved repeatedly with different dual parameters, which increases the computation time significantly. In comparison, the effect of the state augmentation is less critical, since the additional state variable consists of a single scalar that is defined on a compact interval. 
%\textcolor{orange}{Q: Can we actually back this up? I don't think we need to present results in the paper, but it isn't immediately clear to me that 'the effect of the state augmentation is less critical'.} \textcolor{blue}{I agree, this wasn't worded well. What do you think of the new version? -MF} \textcolor{orange}{Sounds good to me - thanks!}
%
%\textcolor{orange}{These values should be regarded as a qualitative comparison of the computation effort required by a naive implementation of each algorithm; no attempt has been made to optimize for computational efficiency beyond leveraging embarrassingly parallelizable operations.}
%Table \ref{tradeoffsbetweenmethods} summarizes the main trade-offs between the state-augmentation and under-approximation methods.
%
%\begin{table}[ht]
%\caption{Trade-offs between Methods}
% \label{table}
%\setlength{\tabcolsep}{3pt}
%\begin{tabular}{|p{120pt}|p{120pt}|}
%\hline
%\textbf{State-Augmentation Method} &  \textbf{Under-Approximation Method \cite{chapmantac2021} }\\
%\hline
%Provides $\mathcal{S}_\alpha^r$ exactly in principle & Provides an under-approximation for $\mathcal{S}_\alpha^r$ in principle \vspace{.5mm}\\
%\hline
%Does not require parameter tuning & The soft-maximum parameter $\gamma$ requires tuning. \vspace{.5mm}\\
%\hline
%Requires significantly more computational resources & Requires significantly less computational resources \vspace{.5mm}\\
%\hline
%Useful for in-depth analysis of a small number of promising designs & Useful as a screening tool to identify more promising designs from a collection of candidate designs \vspace{.5mm}\\
%\hline
%\multicolumn{3}{p{251pt}}{ft $=$ feet, cfs $=$ 
%cubic feet per second.}
%\end{tabular}
%\label{tradeoffsbetweenmethods}
%\end{table}
%
%\subsubsection{Discussion of numerical results} We use the notation $\hat{\mathcal{S}}_\alpha^r$ $(\hat{\mathcal{U}}_{\alpha,\gamma}^r)$ to indicate a computation of $\mathcal{S}_\alpha^r$ $(\mathcal{U}_{\alpha,\gamma}^r)$. This notation emphasizes the distinction between an exact mathematical quantity and a computation of this quantity returned by a computer program. The under-approximation method preserves interesting and potentially useful qualitative features that are provided by the state-augmentation method. For example, the $\hat{\mathcal{S}}_\alpha^r$-contours for the pump design (b) are more rectangular in comparison to those for the baseline design (a) (Fig.~\ref{onlystateaug}). These features are apparent from the $\hat{\mathcal{U}}_{\alpha,\gamma}^r$-contours as well (Fig.~\ref{exactvsunderapprox}, first two rows, pink dotted lines). The $\hat{\mathcal{S}}_\alpha^r$-contours for the outlet design (c) are stretched along the $x_1$-axis in comparison to the baseline design (a) (Fig.~\ref{alldesigns}, top, black vs. pink). This effect is also seen by observing the associated contours of $\hat{\mathcal{U}}_{\alpha,\gamma}^r$ (Fig.~\ref{alldesigns}, bottom, black vs. pink). Increasing the surface area of tank 2 (design d) stretches the contours of $\hat{\mathcal{S}}_\alpha^r$ and $\hat{\mathcal{U}}_{\alpha,\gamma}^r$ along the $x_2$-axis in comparison to the baseline design (Fig.~\ref{alldesigns}, top and bottom, orange dotted vs. pink). As the risk-aversion level $\alpha$ becomes smaller (more pessimistic), the contours of $\hat{\mathcal{S}}_\alpha^r$ and $\hat{\mathcal{U}}_{\alpha,\gamma}^r$ contract, as we expect, while the qualitative features are preserved (Fig.~\ref{exactvsunderapprox}).
%
%While the under-approximation method recovers qualitative features and requires reduced computational resources, it tends to over-estimate the effect of making a design change (Table \ref{comparingdesignstable}). 
%
Consequently, the underapproximation method provides a \emph{preliminary screening} tool to identify more promising designs from a collection of candidate designs. The current method provides a tool for \emph{in-depth analysis} of a small number of promising designs that have been selected through preliminary screening. The risk-aversion level $\alpha$ allows one to specify a degree of pessimism precisely in terms of a fraction of the worst cases. The interpretability and flexibility of $\alpha$ may be useful for assessing trade-offs between system performance and financial considerations in practice, especially given the limited budgets afforded to ``ordinary'' rather than ``safety-critical'' infrastructure.

%\textcolor{blue}{One may ask -- why is $\alpha$ useful? The shapes look similar across alpha...I'd like some help articulating why the risk-aversion level is important -- why it may provide a nuanced interpretation of pessimism, which could be useful for making design choices under uncertainty...want to link the paragraph below better to our numerical results} 
%, which has benefits for designing systems in practice. Stormwater systems are often required to satisfy precise regulatory criteria. For example, an outflow rate must be no more than a given threshold when simulating the outcome from a (non-stochastic) design storm via hydrology and hydraulic modeling software (e.g., \cite{swmm}). Our framework could be used in parallel with standard practices to quantify the effect of stochastic surface runoff on low-dimensional models of proposed designs, as the degree of risk aversion $\alpha$ varies. The value of $\alpha$ provides a systematic and interpretable way to assess a design with respect to varying degrees of pessimism about the future. While the typical minimax approach to control systems leads to robust designs by adopting a worst-case perspective, designing for the worst case may not be financially feasible, especially given the limited budgets afforded to ``ordinary'' rather than ``safety-critical'' infrastructure. Therefore, the flexibility afforded by $\alpha$ may be useful for assessing trade-offs between system performance and financial considerations in practice, given the limited budgets afforded to ``ordinary'' rather than ``safety-critical'' infrastructure.

%\textcolor{orange}{Note: Feel free to adapt the above. My intentions were to basically restate what you had written while avoiding the statement "we would like alpha to be as small as possible" because while I know what you meant, ultimately that is a subjective preference - and the value of CVaR is its ability to accommodate a wide range of such preferences (alpha 0-1). So instead I tried to tie it back to the minimiax control approach introduced in the first line of the paper.} \textcolor{teal}{Sounds good to me. I like the idea of ``closing the circle'' by returning to the argument in opening paragraph. -MF}

%While we would like $\alpha$ to be as small as possible, a design that generates a sufficiently large risk-sensitive safe set for a quite small $\alpha$ may be too expensive to install (e.g., land near urban areas may be expensive).%

%Ultimately, the size of a risk-sensitive safe set for a sufficiently small (but not too small) value of $\alpha$ could define a regulatory criterion that a design must satisfy before it is approved for installation. 
%A designer could balance the desire to choose the smallest (most risk-averse) value of $\alpha$ subject to the (typically fixed) financial budget for the proposed design. financial constraints \textcolor{blue}{....Our framework does xx...However, standard practices do not use a probabilistic model of precipitation...our framework could be used in combination with a high-fidelity computer model in this way...here want to say some vision for how our framework could provide benefits to standard practices, and connect this discussion to the quantitative interpretation of the parameter alpha.}
%
%We consider the effect of different design changes to the system by studying the safe sets across risk-sensitivity levels.
%
%
%exact_vs_underapprox.png
\begin{figure*}[ht]
\centerline{\includegraphics[width=\textwidth]{newvsold_method_3designs.png}}\vspace{-2mm}
\caption{Contours of computations of risk-averse safe sets for $\alpha \in \{0.99, 0.05, 0.005, 0.0005, 5 \cdot 10^{-5}\}$ and $r \in \{0.2, 1, 1.8\}$. Each row pertains to a particular design. Solid blue lines show the numerical results for $\mathcal{S}_\alpha^r$ using \eqref{13}. Pink dotted lines show the numerical results for $\mathcal{U}_{\alpha,\gamma}^r$ ($\gamma = 20$) using the underapproximation method from \cite{chapmantac2021}. We have explored values of $\gamma$ between 10 and 120 in increments of roughly 10. We have chosen $\gamma = 20$ because this value provides relatively large estimates of $\mathcal{U}_{\alpha,\gamma}^r$ for more risk-averse values of $\alpha$. We present the differences between four distinct designs qualitatively and quantitatively in the extended version \cite{extendedversion} of this work. %The selection of an appropriate $\gamma$ depends on one's preferences, and additional guidance is provided in \cite{chapmantac2021}. 
%Computations of risk-sensitive safe sets $\mathcal{S}_\alpha^r$ and under-approximations $\mathcal{U}_{\alpha,\gamma}^r$ for different risk-sensitivity levels $\alpha$ (degree of risk-aversion/pessimism increases from left to right), thresholds $r \in \{0.2, 1, 1.8\}$, and designs. The boundary of $\mathcal{S}_\alpha^r$ is indicated by a black dotted line, and the boundary of $\mathcal{U}_{\alpha,\gamma}^r$ $(\gamma = 22)$ is indicated by a pink solid line. Each row provides sets for a particular design option.
}\vspace{-4mm}
\label{exactvsunderapprox}
\end{figure*}

%\begin{figure*}[ht]
%\centerline{\includegraphics[width=\textwidth]{state_aug_only_2_designs.png}}
%\caption{Contours of computations of risk-averse safe sets for $\alpha \in \{0.99, 0.05, 0.005, 0.0005, 5 \cdot 10^{-5}\}$ and $r \in \{0.1, 0.2, \dots, 1.9\}$ when using the state-augmentation method for two designs: a) baseline and b) replace valve with pump. This figure shows the contour shapes for these two designs in more detail by presenting more values of $r$ compared to Fig.~\ref{exactvsunderapprox}.}
%\label{onlystateaug}
%\end{figure*}

%\begin{figure*}[ht]
%\centerline{\includegraphics[width=\textwidth]{all_designs.png}}
%\caption{This figure presents numerical results from Fig.~\ref{exactvsunderapprox} from a different perspective to depict how a different design may produce a differently shaped or sized contour, $r \in \{0.2, 1, 1.8\}$. We placed the results for all designs in a single sub-plot pertaining to a particular $\alpha$. We used the state-augmentation method to obtain the results in the top row, and the under-approximation method ($\gamma = 20$) to obtain the results in the bottom row. Note that the contours for design a (baseline, magenta solid lines) and design c (add outlet, black solid lines) overlap in regions where $x_2$ has larger values.}
%\label{alldesigns}
%\end{figure*}

%\begin{table}[ht]
%\caption{Quantitative comparison of designs ($r = 1$)}
% \label{table}
%\setlength{\tabcolsep}{3pt}
%\centering
%\begin{tabular}{|p{50pt}|p{50pt}|p{50pt}|p{50pt}|}
%\hline
%\textbf{$\alpha =$ 0.99} &  \textbf{b vs. a} &  \textbf{c vs. a} & \textbf{d vs. a} \vspace{.5mm}\\
%\hline
%State-Aug & 0.93 & 0.079 & 0.34\vspace{.5mm}\\
%Under-Approx. & 2.6 & 0.069 & 0.93\vspace{.5mm}\\
%\hline
%\textbf{$\alpha =$ 0.05} &  \textbf{b vs. a} &  \textbf{c vs. a} & \textbf{d vs. a} \vspace{.5mm}\\
%\hline
%State-Aug & 2.1 & 0.068 & 0.71\vspace{.5mm}\\
%Under-Approx. & 3.6 & 0.059 & 1.3\vspace{.5mm}\\
%\hline
%\textbf{$\alpha =$ 0.005} &  \textbf{b vs. a} &  \textbf{c vs. a} & \textbf{d vs. a} \vspace{.5mm}\\
%\hline
%State-Aug & 3.1 & 0.059 & 1.1\vspace{.5mm}\\
%Under-Approx. & 5.1 & 0.072 & 1.9\vspace{.5mm}\\
%\hline
%\textbf{$\alpha =$ 0.0005} &  \textbf{b vs. a} &  \textbf{c vs. a} & \textbf{d vs. a} \vspace{.5mm}\\
%\hline
%State-Aug & 4.9 & 0.055 & 1.8\vspace{.5mm}\\
%Under-Approx. & 7.6 & 0.03 & 2.8\vspace{.5mm}\\
%\hline
%\textbf{$\alpha =$ 0.00005} &  \textbf{b vs. a} &  \textbf{c vs. a} & \textbf{d vs. a} \vspace{.5mm}\\
%\hline
%State-Aug & 9.0 & 0.054 & 3.3\vspace{.5mm}\\
%Under-Approx. & 14 & 0.031 & 5.3\vspace{.5mm}\\
%\hline
%\multicolumn{4}{p{230pt}}{We list the increase in the size of a risk-averse safe set for design b, c, or d compared to the baseline (design a). This is a quantitative depiction of the some of the results in Fig.~\ref{alldesigns}. Let $\text{N}_{\text{y},\alpha}$ denote the number of states in the computation of $\mathcal{S}_\alpha^r$ for design y $\in \{\text{a},\text{b},\text{c},\text{d}\}$ and $r = 1$. Let $\hat{\text{N}}_{\text{y},\alpha}$ denote the number of states in the computation of $\mathcal{U}_{\alpha,\gamma}^r$ for design y, $r = 1$, and $\gamma = 20$. Each quantity in a row labeled State-Aug takes the form: $(\text{N}_{\text{y},\alpha}-\text{N}_{\text{a},\alpha})/\text{N}_{\text{a},\alpha}$. Each quantity in a row labeled Under-Approx. takes the form: $(\hat{\text{N}}_{\text{y},\alpha}-\hat{\text{N}}_{\text{a},\alpha})/\hat{\text{N}}_{\text{a},\alpha}$.}
%\end{tabular}
%\label{comparingdesignstable}
%\end{table}



